Metadata-private Messaging without Coordination

For those seeking end-to-end private communication free from pervasive metadata tracking and censorship, the Tor network has been the de-facto choice in practice, despite its susceptibility to traffic analysis attacks. Recently, numerous metadata-private messaging proposals have emerged with the aim to surpass Tor in the messaging context by obscuring the relationships between any two messaging buddies, even against global and active attackers. However, most of these systems face an undesirable usability constraint: they require a metadata-private "dialing" phase to establish mutual agreement and timing or round coordination before initiating any regular chats among users. This phase is not only resource-intensive but also inflexible, limiting users' ability to manage multiple concurrent conversations seamlessly. For stringent privacy requirement, the often-enforced traffic uniformity further exacerbated the limitations of this roadblock. In this paper, we introduce PingPong, a new end-to-end system for metadata-private messaging designed to overcome these limitations. Under the same traffic uniformity requirement, PingPong replaces the rigid "dial-before-converse" paradigm with a more flexible "notify-before-retrieval" workflow. This workflow incorporates a metadata-private notification subsystem, Ping, and a metadata-private message store, Pong. Both Ping and Pong leverage hardware-assisted secure enclaves for performance and operates through a series of customized oblivious algorithms, while meeting the uniformity requirements for metadata protection. By allowing users to switch between conversations on demand, PingPong achieves a level of usability akin to modern instant messaging systems, while also offering improved performance and bandwidth utilization for goodput. We have built a prototype of PingPong with 32 8-core servers equipped with enclaves to validate our claims.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> olddraft.tex <==


\begin{figure}
\begin{tcolorbox}[
    enhanced,
    colback=white, % Background color
    colframe=black, % Border color
    %arc=0mm, % Border radius
    boxrule=1pt, % Border thickness
    left=2pt, % Left margin
    right=2pt, % Right margin
    top=2pt, % Top margin
    bottom=2pt, % Bottom margin
    %fontupper=\small,
   % breakable % Allow box to break across pages
  ]

%\noindent\textbf{Input:} the security parameter $\lambda$, the maximum round of messages $N$, the maximum batch size $c$.
\underline{$\mathsf{notf\_pkt} \leftarrow \texttt{GenNotf}(\mathsf{Buddy\_ID}, sk_{encl})$:} 
\begin{algorithmic}[1]
\State Initialize a binary bit vector $\mathsf{notf\_vec} = 0^n$, where $n$ is the maximum contact size. 
\State $\mathsf{frd\_ind} = \texttt{FriendList.getIndex}(\mathsf{ID}=\mathsf{Buddy\_ID})$ 
\State $\mathsf{carrier\_label} = \texttt{FriendList}[\mathsf{frd\_ind}].\mathsf{label}$ 

\State $\mathsf{notf\_vec}[\mathsf{frd\_ind}] = 1$ 

\State $\mathsf{notf\_pkt} \leftarrow \texttt{Encrypt}(\mathsf{carrier\_label}||\mathsf{notf\_vec},sk_{encl})$

\State  \textbf{Return} $\mathsf{notf\_pkt}$
%
\end{algorithmic}
%
%
\underline{$\mathsf{msg\_pkt} \leftarrow \texttt{GenMsg}(\mathsf{Buddy\_ID}, \mathsf{data}, sk_{encl})$:} 
\begin{algorithmic}[1]
\State $\mathsf{frd\_ind} = \texttt{FriendList.getIndex}(\mathsf{ID}=\mathsf{Buddy\_ID})$ 
\State $sk =\texttt{FriendList}[\mathsf{frd\_ind}].sk$
\State \Comment{Generate message token}
\State $\mathsf{counter} = \texttt{FriendList}[\mathsf{frd\_ind}].\mathsf{counter}_s$
\State $\mathsf{token} = \texttt{PRF}_{sk}(\mathsf{Buddy\_ID}||\mathsf{My\_ID}||\mathsf{counter})$
\State $\texttt{FriendList}[\mathsf{frd\_ind}].\mathsf{counter}_s++$
\State \Comment{Encrypt message content}
\State $\mathsf{data\_pkt}\leftarrow \texttt{Encrypt}(\mathsf{My\_ID}||\texttt{Encrypt}(\mathsf{data},sk),sk_{encl})$

\State $\mathsf{msg\_pkt} \leftarrow \texttt{Encrypt}(\mathsf{token}||\mathsf{data\_pkt},sk_{encl})$


\State  \textbf{Return} $\mathsf{msg\_pkt}$
%
\end{algorithmic}
%$$
%%
\underline{$\mathsf{msg\_tokens} \leftarrow \texttt{ParseNotf}(\mathsf{notf\_vec})$:} 
%
\begin{algorithmic}[1]
\For { $b \in 1...\texttt{len}(\mathsf{notf\_vec})$}
\If {$\mathsf{notf\_vec}[b] = 1$}
\State $\mathsf{Buddy\_ID} = \texttt{FriendList}[b].\mathsf{ID}$
\State $\mathsf{counter} = \texttt{FriendList}[b].\mathsf{counter}_r$
\State $sk =\texttt{FriendList}[b].sk$
\State $\mathsf{token} = \texttt{PRF}_{sk}(\mathsf{My\_ID}||\mathsf{Buddy\_ID}||\mathsf{counter})$
\State $\texttt{FriendList}[b].\mathsf{counter}_r++$
\State Append $\mathsf{token}$ to $\mathsf{msg\_tokens}$
\EndIf
\EndFor
\State  \textbf{Return} $\mathsf{msg\_tokens}$
\end{algorithmic}
\end{tcolorbox}
  \caption{Pseudocode for functions of generating and parsing notification and message packets (client local operations).}
    \label{fig:clientfunccode}
\end{figure}


\begin{figure}
\begin{tcolorbox}[
    enhanced,
    colback=white, % Background color
    colframe=black, % Border color
    %arc=0mm, % Border radius
    boxrule=1pt, % Border thickness
    left=2pt, % Left margin
    right=2pt, % Right margin
    top=2pt, % Top margin
    bottom=2pt, % Bottom margin
    %fontupper=\small,
   % breakable % Allow box to break across pages
  ]

\underline{Sending thread:} 

%\noindent\textbf{Input:} the write batch $\mathsf{W} = \{k_i, v_i\}_{i = 1...n\leq c}$ and the hierarchichal OHTs $\tilde{\textbf{T}}$.
\begin{algorithmic}[1]

\While {\pythoninline{True}}
\If {idle}
\State $\mathsf{notf\_pkt} \leftarrow \texttt{GenNotf}(\mathsf{0}, sk_{encl})$
\State $\mathsf{msg\_pkt} \leftarrow  \texttt{Encrypt}(\perp ||~\text{random()},sk_{encl})$
\Else
\State $\mathsf{notf\_pkt} \leftarrow \texttt{GenNotf}(\mathsf{Buddy\_ID}, sk_{encl})$
 \State $\mathsf{msg\_pkt} \leftarrow \texttt{GenMsg}(\mathsf{Buddy\_ID}, \mathsf{content},sk_{encl})$
\EndIf
  \State  (rpc call) $ \texttt{SendNotf}(\mathsf{notf\_pkt})$
  \State (rpc call) $ \texttt{SendMsg}(\mathsf{msg\_pkt})$
\EndWhile
\end{algorithmic}

\underline{Receiving thread:} 

%\noindent\textbf{Input:} the write batch $\mathsf{W} = \{k_i, v_i\}_{i = 1...n\leq c}$ and the hierarchichal OHTs $\tilde{\textbf{T}}$.
\begin{algorithmic}[1]

\While {\pythoninline{True}}
  \State (rpc call) $\mathsf{notf\_pkt} \leftarrow  \texttt{RecvNotf}()$ 
  \State  $\mathsf{notf\_vec} \leftarrow \texttt{Decrypt}(\mathsf{notf\_pkt},sk_{encl})$
\State $\mathsf{msg\_tokens} \leftarrow \texttt{ParseNotf}(\mathsf{notf\_vec})$
\For{$\mathsf{msg\_token} \in \mathsf{msg\_tokens}$}
  \State $\mathsf{req\_pkt} = \texttt{Encrypt}(\mathsf{msg\_token},sk_{encl}) $
  \State (rpc call) $\mathsf{data\_pkt}\leftarrow \texttt{SendRequest}(\mathsf{req\_pkt})$ 
  \State $\mathsf{Buddy\_ID}, \mathsf{enc\_data} \leftarrow \texttt{Decrypt}(\mathsf{data\_pkt},sk_{encl})$
  \State Lookup the secret key from $ \texttt{FriendList}$ and decrypt $\mathsf{enc\_data}$.
\EndFor
\EndWhile
\end{algorithmic}

\end{tcolorbox}
  \caption{Client main loop.}
    \label{fig:clientloop}
\end{figure}






\begin{algorithmic}
  \State \textbf{Local APIs:}
  \State $\mathsf{my\_ind}, \mathsf{priv\_label}, sk, \mathsf{ctr} \leftarrow \texttt{GetContact}(\mathsf{Buddy\_ID})$
  \State $\mathsf{notf\_pkt} \leftarrow \texttt{GenNotf}(\mathsf{Buddy\_ID}, sk_{encl})$
  \State $\mathsf{notf\_pkt} \leftarrow \texttt{RecvNotf}()$
  \State $\mathsf{msg\_token} \leftarrow \texttt{ParseNotf}(\mathsf{notf\_msg})$
  \State $\mathsf{msg\_pkt} \leftarrow \texttt{GenMsg}(\texttt{FriendList}, \mathsf{Buddy\_ID}, \mathsf{msg\_content})$


  \State \textbf{Client-server interaction APIs:}
  \State $ \cdot \leftarrow \texttt{SendNotf}(\mathsf{notf\_pkt})$
  \State $\mathsf{notf\_pkt} \leftarrow \texttt{RecNotf}(\mathsf{Client\_ID})$ 
  \State $ \cdot \leftarrow \texttt{SendMsg}(\mathsf{msg\_token_{cipher}}, \mathsf{msg\_pkt})$
  \State $\mathsf{msg\_pkt}\leftarrow \texttt{RetrieveMsg}(\mathsf{msg\_token_{cipher}})$ 

\end{algorithmic}
\end{tcolorbox}
  \caption{\name{}'s APIs.}
    \label{fig:APIs}
\end{figure}

\begin{figure}[ht]
\centering
\begin{tcolorbox}[
    enhanced,
    colback=white, % Background color
    colframe=black, % Border color
    %arc=0mm, % Border radius
    boxrule=1pt, % Border thickness
    left=2pt, % Left margin
    right=2pt, % Right margin
    top=0pt, % Top margin
    bottom=0pt, % Bottom margin
    %fontupper=\small,
   % breakable % Allow box to break across pages
  ]
\begin{lstlisting}[basewidth=0.5em]
// Initialize an Alpenhorn account
func Register(email string)

// Get your long-term key to share with friends
func MySigningKey() PublicKey

// Send friend request to the given email address.
// Their public key for extra verification is optional.
func AddFriend(email string, theirSigningKey *PublicKey)

// Call a friend; returns a shared secret known only
// to you and the friend. The call's intent is optional.
func Call(email string, intent int) SessionKey
\end{lstlisting}
\end{tcolorbox}
\caption{Simplified Alpenhorn API}
\label{fig:alpenhornapi}
\end{figure}







\begin{figure}
\begin{tcolorbox}[
    enhanced,
    colback=white, % Background color
    colframe=black, % Border color
    %arc=0mm, % Border radius
    boxrule=1pt, % Border thickness
    left=2pt, % Left margin
    right=2pt, % Right margin
    top=2pt, % Top margin
    bottom=2pt, % Bottom margin
    %fontupper=\small,
   % breakable % Allow box to break across pages
  ]
\underline{\name{}'s API:} 

%\noindent\textbf{Input:} the security parameter $\lambda$, the maximum round of messages $N$, the maximum batch size $c$.

\begin{algorithmic}
  \State \textbf{Local APIs:}
  \State $\mathsf{my\_ind}, \mathsf{priv\_label}, sk, \mathsf{ctr} \leftarrow \texttt{GetContact}(\mathsf{Buddy\_ID})$
  \State $\mathsf{notf\_pkt} \leftarrow \texttt{GenNotification}(\mathsf{Buddy\_ID}, sk_{encl})$
  \State $\mathsf{notf\_pkt} \leftarrow \texttt{RecvNotification}()$
  \State $\mathsf{msg\_token} \leftarrow \texttt{ParseNotification}(\mathsf{notf\_msg})$
  \State $\mathsf{msg\_pkt} \leftarrow \texttt{GenMsg}(\texttt{FriendList}, \mathsf{Buddy\_ID}, \mathsf{msg\_content})$


  \State \textbf{Client-server interaction APIs:}
  \State $ \cdot \leftarrow \texttt{SendNotification}(\mathsf{notf\_pkt})$
  \State $\mathsf{notf\_pkt} \leftarrow \texttt{RecNotification}(\mathsf{Client\_ID})$ 
  \State $ \cdot \leftarrow \texttt{SendMsg}(\mathsf{msg\_token_{cipher}}, \mathsf{msg\_pkt})$
  \State $\mathsf{msg\_pkt}\leftarrow \texttt{RetrieveMsg}(\mathsf{msg\_token_{cipher}})$ 

\end{algorithmic}
\end{tcolorbox}
  \caption{\name{}'s APIs.}
    \label{fig:APIs}
\end{figure}
